An Emerging Coherent Picture of Red Supergiant Supernova Explosions

Three lines of evidence indicate that in the most common type of core collapse supernovae, the energy deposited in the ejecta by the exploding core is approximately proportional to the progenitor mass cubed. This results stems from an observed uniformity of light curve plateau duration, a correlation between mass and ejecta velocity, and the known correlation between luminosity and velocity. This result ties in analytical and numerical models together with observations, providing us with clues as to the mechanism via which the explosion of the core deposits a small fraction of its energy into the hurled envelope.

==> tbl1.tex <==

 
\begin{deluxetable}{lcl}\label{t:1}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{SN name} &
\colhead{M (M$_{\odot}$)} &
\colhead{Source}}
\tablecaption{Masses}
\startdata
1999an & $<\,18$ & \cite{smartt09} \\ 
1999br & $<\,15$ & \cite{smartt09} \\ 
1999em & $<\,15$ & \cite{smartt09} \\ 
1999gi & $<\,14$ & \cite{smartt09} \\ 
2001du & $<\,15$ & \cite{smartt09} \\ 
2002hh & $<\,18$ & \cite{smartt09} \\ 
2003gd & $ 8^{+2}_{-2}$ & \cite{maund13} \\ 
2003ie & $<\,25$ & \cite{smartt09} \\ 
2004A & $12^{+2}_{-2}$ & \cite{maund13} \\ 
2004am & $12^{+7}_{-3}$ & \cite{smartt09} \\ 
2004dg & $<\,12$ & \cite{smartt09} \\ 
2004dj & $15^{+3}_{-3}$ & \cite{smartt09} \\ 
2004et & $11^{+2}_{-1}$ & \cite{jerkstrand12} \\ 
2005cs & $10^{+3}_{-2}$ & \cite{maund13} \\ 
2006bc & $<\,12$ & \cite{smartt09} \\ 
2006my & $10^{+2}_{-2}$ & \cite{maund13} \\ 
2006ov & $<\,11$ & \cite{smartt09} \\ 
2007aa & $<\,12$ & \cite{smartt09} \\ 
2008bk & $ 9^{+4}_{-1}$ & \cite{smartt09} \\ 
2009kr & $21^{+3}_{-3}$ & \cite{elias-rosa10} \\ 
2009md & $ 8^{+6}_{-1}$ & \cite{fraser11} \\ 
2012aw & $18^{+2}_{-2}$ & \cite{van-dyk12} \\ 
2012ec & $18^{+4}_{-4}$ & \cite{maund13a} \\ 
\enddata
\end{deluxetable}

